Study of the High Energy Gamma-ray Emission from the Crab Pulsar with the MAGIC telescope and Fermi-LAT

My thesis deals with a fundamental question of high energy gamma-ray astronomy. Namely, I studied the cut-off shape of the Crab pulsar spectrum to distinguish between the leading scenarios for the pulsar models. Pulsars are celestial objects, which emit periodic pulsed electromagnetic radiation (pulsation) from radio to high energy gamma-rays. Two major scenarios evolved in past 40 years to explain the pulsation mechanism: the inner magnetosphere scenario and the outer magnetosphere scenario. Both scenarios predict a high energy cut-off in the gamma-ray energy spectrum, but with different cut-off sharpness. An exponential cut-off is expected for the outer magnetosphere scenario while a super-exponential cut-off is predicted for the inner magnetosphere scenario. Therefore, one of the best ways to confirm or rule out these scenarios is to measure the energy spectrum of a pulsar at around the cut-off energy, i.e., at energies between a few GeV and a few tens of GeV. All past attempts (>10) to measure pulsars with ground-based instruments have failed while satellite-borne detectors had a too small area to study detailed spectra in the GeV domain. In this thesis, the gamma-ray emission at around the cut-off energy from the Crab pulsar is studied with the MAGIC telescope. The public data of the satellite-borne gamma-ray detector, Fermi-LAT, are also analyzed in order to discuss the MAGIC observation results in comparison with the adjacent energy band.

==> UnitsEtc.tex <==
%\addcontentsline{toc}{chapter}{\protect Zusammenfassung}
\chapter*{List of Acronyms and Abbreviations}
\begin{table}[h]
\begin{tabular}{ll}
AGASA & Akeno Giant Air Shower Array \\
AGN & Active Galactic Nuclei \\
a.s.l. & above sea level \\
BeppoSAX & Satellite per Astronomia X ("Beppo" in honor of Giuseppe Occhialini) \\
CANGAROO & Collaboration of Australia and Nippon (Japan) for a GAmma Ray Observatory \\
 & in the Outback \\
CCD & Charge-Coupled Device \\
CE & Collection Efficiency \\
CGRO & Compton Gamma-Ray Observatory \\
CIB  & Cosmic Infrared Background \\
CMB  & Cosmic Microwave Background \\
COB  & Cosmic Optical Background \\
COG & Center Of Gravity \\
COMPTEL & imaging COMPton TELescope (on CGRO)\\
CR & Cosmic Ray \\
CTA & Cherenkov Telescope Array \\
DAQ & Data AcQuisition \\
dof & degree of freedom \\
EBL & Extragalactic Background Light \\
EGRET & Energetic Gamma-Ray Experiment Telescope (on CGRO) \\
FADC & Flash Analogue-to-Digital Converter \\
FoV & Field of View \\
FWHM & Full Width Half Maximum \\
GRB & Gamma-Ray Burst \\
GBM  & Gamma-ray Burst Monitor (on \fermi~gamma-ray space telescope)  \\
GPS & Global Positioning System \\
GZK & Greisen-Zatsepin-Kuzmin \\
HESS & High Energy Stereoscopic System \\
HiRes & High Resolution fly's eye \\ 
HRI &  High Resolution Imager \\
HV & High Voltage \\
\end{tabular}
\end{table}
\begin{table}[h]
\begin{tabular}{ll}
IR & InfraRed \\ 
IACT & Imaging Atmospheric Cherenkov Telescope \\
LAT  & Large Area Telescope (on \fermi~gamma-ray space telescope)  \\
LED  & Light Emitting Diode \\
MAGIC & Major Atmospheric Gamma-ray Imaging Cherenkov telescope \\
MECS & Medium Energy Concentrator Spectrometer \\
MC   & Monte Carlo simulation\\
MJD  & Modified Julian Day\\
MSSM & Minimal Supersymmetric Standard Model \\
NN & Next Neighboring \\ 
NSB  & Night Sky Background\\
OG & Outer Gap \\
PC & Polar Cap \\
PDE & Photodetection Efficiency \\ 
PFF & Pair Formation Front \\
ph.e. & PhotoElectron \\ 
PCB & Print Circuit Board \\
PDS & Phoswich Detector System \\
PMT & PhotoMulitiplier Tube \\
PSF & Point Spread Function \\ 
PSR & Pulsar \\
PWN & Pulsar Wind Nebula \\
QCD & Quantum ChromoDynamics \\
QE & Quantum Efficiency \\
QG & Quantum Gravity \\
RMS & Root Mean Square \\
ROSAT & R$\ddot{\rm O}$ntgenSATellit \\
SCLF & Space Charge Limited Flow \\
SED  & Spectral Energy Distribution \\
SG & Slot Gap \\
SMBH & SuperMassive Black Hole \\
SNR & SuperNova Remnant \\
SUSY & SUperSYmmetry \\
UV & UltraViolet \\ 
VCSEL & Vertical-Cavity Surface-Emitting Laser \\
VERITAS & Very Energetic Radiation Imaging Telescope Array System \\ 
VHE  & Very High Energy ($>$10 GeV) \\
WIMP & Weakly Interacting Massive Particle \\
WLS & WaveLength Shifter \\
WMAP & Wilkinson Microwave Anisotropy Probe \\
WR & Wolf-Rayet \\
ZA & Zenith Angle \\
\end{tabular}
\end{table}
\chapter*{List of Useful Units}
%\clearpage
%{\Huge \bf List of Useful Units} 
In addition to the standard units in the cgs system, following units are useful in astrophysics and
will be used in this thesis.
\begin{table}[h]
\begin{tabular}{ll}
eV  & $ 1.602 \times 10^{-12}$ erg \\
keV & $10^3$ eV \\
MeV & $10^6$ eV \\
GeV & $10^9$ eV \\
TeV & $10^{12}$ eV \\
PeV & $10^{15}$ eV \\
pc  & $3.086 \times 10^{18}$ cm\\
kpc  & $10^3$ pc \\
Mpc  & $10^6$ pc \\
b & $10^{-24}$ cm$^{-2}$ \\
mb & $10^{-3}$ b
\end{tabular}
\end{table}
%\clearpage
%\chapter*{List of Useful Physics Constants and Parameters}
%\\
\\
{\LARGE \bf List of Useful Physics Constants and Parameters}
\\
\begin{table}[h]
\begin{tabular}{lll}
$c$  & speed of light & $2.998 \times 10^{10}$ cm/s \\
$h$  & Planck constant & $6.602 \times 10^{-27}$ erg s \\
$\hbar$  & = $h/2\pi$, reduced Planck constant & $1.054 \times 10^{-27}$ erg s \\
$G$  & Newtonian gravitational constant & $6.6742 \times 10^{-8}$ cm$^{3}$ g$^{-1}$ s$^{-2}$ \\
& \\
$e$  & electric charge of an electron & $4.803 \times 10^{-10}$ esu, $1.602 \times 10^{-19}$ C \\ 
$m_e$ & mass of an electron & $9.109 \times 10^{-28}$ g, 511 keV/c$^2$ \\
$m_\mu$ & mass of muon & 105.7 MeV/c$^2$ \\
%$m_p$ & mass of proton & 938.3 MeV/c$^2$ \\
$m_{\pi_0}$ & mass of a neutral pion & 134.98 MeV/c$^2$ \\
$\alpha$ & $= e^2/\hbar c$, fine structure constant & $7.297 \times 10^{-3}$ = 1/137.035  \\
$r_e $ & $= e^2/m_e c^2$, classical electron radius & $2.818 \times 10^{-13}$ cm \\
$\sigma_T $ & $= 8\pi r_e^2/3$, Thomson cross section & $6.652 \times 10^{-25}$ cm$^2$ \\
$\lambda \hspace{-0.5em}\raisebox{0.5ex}{--} $ & $= \hbar/m_e c = r_e/\alpha$, electron Compton wavelength & $3.862 \times 10^{-11}$ cm \\
$B_c $ & $= m_e^2c^3/\hbar e$, critical magnetic field strength & $4.414 \times 10^{13}$ G \\
$M_\odot$ & solar mass & $1.988 \times 10^{33}$ g 
\end{tabular}
\end{table}

